A Logical Fallacy-Informed Framework for Argument Generation

Despite the remarkable performance of Large Language Models (LLMs) in natural language processing tasks, they still struggle with generating logically sound arguments, resulting in potential risks such as spreading misinformation. To address this issue, we introduce FIPO, a fallacy-informed framework that leverages preference optimization methods to steer LLMs toward logically sound arguments. FIPO includes a classification loss, to capture the fine-grained information on fallacy types. Our results on argumentation datasets show that our method reduces the fallacy errors by up to 17.5%. Furthermore, our human evaluation results indicate that the quality of the generated arguments by our method significantly outperforms the fine-tuned baselines, as well as other preference optimization methods, such as DPO. These findings highlight the importance of ensuring models are aware of logical fallacies for effective argument generation. Our code is available at github.com/lucamouchel/Logical-Fallacies.

==> figures/portion_train_val_test.tex <==
\begin{tikzpicture}

% Data
\def\trainTotal{8918}
\def\validTotal{0}
\def\testTotal{1319}

\def\trainOriginal{1968}
\def\validOriginal{0}
\def\testOriginal{400}

\def\trainGenerated{6950}
\def\validGenerated{0}
\def\testGenerated{919}

% Following are something we could want to change, such as colors, the legend, the circle size, etc. 
% Color definitions
\definecolor{trainColor}{HTML}{6495ED} % Cornflower Blue
\definecolor{validationColor}{HTML}{B0E0E6} % Powder Blue
\definecolor{testColor}{HTML}{FFDEAD} % Navajo White
\definecolor{originalColor}{HTML}{8FBC8F} % Dark Sea Green
\definecolor{generatedColor}{HTML}{D2B48C} % Tan

% Parameters for the radii of the circles
\def\innerRadius{1.5}
\def\middleRadius{3}
\def\outerRadius{4.5}
% Legend
\node[align=left, font=\small] at (4.5, -3.5) {
    % \textbf{Legend:}\\
    \tikz\draw[originalColor, fill=originalColor] (0,0) rectangle (3ex,1ex); Original \\
    \tikz\draw[generatedColor, fill=generatedColor] (0,0) rectangle (3ex,1ex); Generated
};


% Draw dividing lines for clarity
% \draw[thick] (0,0) -- (\trainAngle:\outerRadius);
% \draw[thick] (0,0) -- (\trainAngle + \validAngle:\outerRadius);
% \draw[thick] (0,0) -- (360:\outerRadius);

% Annotations
\node at (120:2) {Train};
\node at (283:2) {Validation};
\node at (342:2) {Test};

%%%%%%%%%%%%%%%  Following are some plot techniques.  %%%%%%%%%%%%%%%
% Calculate total
\pgfmathsetmacro{\total}{\trainTotal + \validTotal + \testTotal}

% Calculate angles for Train, Validation, Test
\pgfmathsetmacro{\trainAngle}{\trainTotal / \total * 360}
\pgfmathsetmacro{\validAngle}{\validTotal / \total * 360}
\pgfmathsetmacro{\testAngle}{\testTotal / \total * 360}

% Calculate sub-angles for Original and Generated in each segment
\pgfmathsetmacro{\trainOriginalAngle}{\trainOriginal / \trainTotal * \trainAngle}
\pgfmathsetmacro{\trainGeneratedAngle}{\trainGenerated / \trainTotal * \trainAngle}

%\pgfmathsetmacro{\validOriginalAngle}{\validOriginal / \validTotal * \validAngle}
%\pgfmathsetmacro{\validGeneratedAngle}{\validGenerated / \validTotal * \validAngle}

\pgfmathsetmacro{\testOriginalAngle}{\testOriginal / \testTotal * \testAngle}
\pgfmathsetmacro{\testGeneratedAngle}{\testGenerated / \testTotal * \testAngle}






\fill[trainColor] (0,0) -- (0:\middleRadius) arc (0:\trainAngle:\middleRadius) -- cycle;
\fill[originalColor] (0: \middleRadius) arc (0:\trainOriginalAngle:\middleRadius) -- (\trainOriginalAngle:\outerRadius) arc (\trainOriginalAngle:0:\outerRadius) -- cycle;
\fill[generatedColor] (\trainOriginalAngle: \middleRadius) arc (\trainOriginalAngle:\trainAngle:\middleRadius) -- (\trainAngle:\outerRadius) arc (\trainAngle:\trainOriginalAngle:\outerRadius) -- cycle;

% Validation Segment
\fill[validationColor] (0,0) -- (\trainAngle:\middleRadius) arc (\trainAngle:\trainAngle + \validAngle:\middleRadius) -- cycle;
\fill[originalColor] (\trainAngle: \middleRadius) arc (\trainAngle:\trainAngle + \validOriginalAngle:\middleRadius) -- (\trainAngle + \validOriginalAngle:\outerRadius) arc (\trainAngle + \validOriginalAngle:\trainAngle:\outerRadius) -- cycle;
\fill[generatedColor] (\trainAngle + \validOriginalAngle: \middleRadius) arc (\trainAngle + \validOriginalAngle:\trainAngle + \validAngle:\middleRadius) -- (\trainAngle + \validAngle:\outerRadius) arc (\trainAngle + \validAngle:\trainAngle + \validOriginalAngle:\outerRadius) -- cycle;

% Test Segment
\fill[testColor] (0,0) -- (\trainAngle + \validAngle:\middleRadius) arc (\trainAngle + \validAngle:\trainAngle + \validAngle + \testAngle:\middleRadius) -- cycle;
\fill[originalColor] (\trainAngle + \validAngle: \middleRadius) arc (\trainAngle + \validAngle:\trainAngle + \validAngle + \testOriginalAngle:\middleRadius) -- (\trainAngle + \validAngle + \testOriginalAngle:\outerRadius) arc (\trainAngle + \validAngle + \testOriginalAngle:\trainAngle + \validAngle:\outerRadius) -- cycle;
\fill[generatedColor] (\trainAngle + \validAngle + \testOriginalAngle: \middleRadius) arc (\trainAngle + \validAngle + \testOriginalAngle:\trainAngle + \validAngle + \testAngle:\middleRadius) -- (\trainAngle + \validAngle + \testAngle:\outerRadius) arc (\trainAngle + \validAngle + \testAngle:\trainAngle + \validAngle + \testOriginalAngle:\outerRadius) -- cycle;

% Inner White Circle
\fill[white] (0,0) circle (\innerRadius);
% Annotations
\node at (120:2) {Train};
\node at (283:2) {};
\node at (342:2) {Test};



\end{tikzpicture}
